CRLLK: Constrained Reinforcement Learning for Lane Keeping in Autonomous Driving

Lane keeping in autonomous driving systems requires scenario-specific weight tuning for different objectives. We formulate lane-keeping as a constrained reinforcement learning problem, where weight coefficients are automatically learned along with the policy, eliminating the need for scenario-specific tuning. Empirically, our approach outperforms traditional RL in efficiency and reliability. Additionally, real-world demonstrations validate its practical value for real-world autonomous driving.

==> contents/background.tex <==
\section{Background}
\label{sec:bck}
\vskip 4pt
% \subsection{Markov Decision Process:}
\noindent\textbf{Markov Decision Process.} We formally describe the LK problem with a Markov decision process (MDP)~\cite{puterman2014markov}. An MDP is defined by a tuple $\langle \mc S, \mc A, \mc T, r, \gamma, H \rangle$, where $s_t \in \mc S$ is a state of the environment, and $a_t \in \mc A$ denotes the action of the agent. At each time step $t$, the environment transitions to a next state $s_{t+1}$ according to a probabilistic transition function $\mc T(s_{t+1} | s_t, a_t)$ after execution of action $a_t$ at state $s_t$. The agent then receives a reward $r(s_t, a_t)$ from the environment for taking action $a_t$ in state $s_t$. $\gamma \in [0, 1)$ is a discount factor and $H$ is a planning horizon. The agent gets action $a_t$ from a parameterized policy $\pi_\theta(\cdot|s_t)$ with parameter $\theta$. The goal is to find a policy $\pi_\theta$ that maximizes the expected value of the objective,
\begin{equation}
\max_{\pi_\theta \in \Pi} J_R^{\pi_\theta}, \text{ where } J_R^{\pi_\theta} = \E \left[ \sum_{t=0}^{H-1} \gamma^t \cdot r(s_t, a_t) | \pi_\theta \right]
\label{eq:mdp}
\end{equation}

% \vskip 2pt
\noindent\textbf{Constrained Markov Decision Process.} A constrained Markov decision process (CMDP)~\cite{Altman98} is an extension of MDP augmented with cost functions. Like the reward function $r(s_t, a_t)$, cost function $c(s_t, a_t)$ also depends on the state-action pair $(s_t, a_t)$. A constraint $C(s_t) = F(c(s_t, a_t), \ldots, c(s_{H-1}, a_{H-1}))$ is also defined on the cost functions, and generally, it can be either in the form of an average or a discounted sum. The objective in CMDP is not only to maximize the long-term discounted reward $J_R^{\pi_\theta}$ as in Equation~\eqref{eq:mdp}, but also to keep the constraint within a threshold value. The overall constrained optimization problem becomes,
\begin{align}
\max_{\pi_\theta \in \Pi} J_R^{\pi_\theta}, \;\; s.t.\;\; J_{C}^{\pi_\theta} \leq \alpha
\label{eq:cmdp}
\end{align}
where, $J_{C}^{\pi_\theta} = \E[C(s_t)]$ and $\alpha$ is a real number.

\vskip 4pt
\noindent\textbf{Duckietown Environment:} A state $s_t$ in the LK problem is an RGB image from the Duckiebot’s monocular camera in both simulation and real-world settings. An action $a_t$ controls the Duckiebot's wheel speeds%, with further details provided in Section~\ref{sec:experiments}
. The reward $r(s, a) $ and cost functions $c(s, a)$ are defined in the next section. More details on Duckietown framework are provided in the Appendix.
% \noindent\textbf{Duckietown Environment:} We briefly describe the Duckietown environment. A state $s_t$ in the LK problem is an RGB image captured by the Duckiebot’s monocular camera in both simulation and real-world settings. An action $a_t$ corresponds to the wheel speeds of the Duckiebot\gao{, with further setting details provided in Section~\ref{sec:experiments}.} The definitions of the reward $r(s, a) $ and cost functions $c(s, a)$ are provided in the next section. More details on Duckietown framework are provided in Appendix.
% \aea{This seems incomplete. What are the actions in the discrete and continuous worlds?(done)}
% \textcolor{blue}{further details are provided in Appendix 1.1. The probabilistic transition function $\mc T$ is the dynamic, modeling how the Duckiebot’s actions affect its movement and subsequent visual observations. The formulation of the reward function  $r$ is present in Section \ref{sec:methodology}.}



==> contents/endorsement.tex <==
\section*{Supervisor Endorsement}

I am pleased to endorse the contributions of Gangadhar Royyuru and Michael Yuhas to the project, \textit{CRLLK: Constrained Reinforcement Learning for Lane Keeping in Autonomous Driving}.

Gangadhar Royyuru, a student at the Indian Institutes of Technology (IIT), was pivotal in developing and implementing the discrete baseline experiments, as well as conducting detailed testing and data analysis. Michael Yuhas, a PhD student, made a significant impact on implementing the real-world experiments and demonstrations.

Their collaboration with the broader team was instrumental in refining the methodology, interpreting the results, and drafting the manuscript. Both students demonstrated a high level of dedication and technical expertise, which contributed meaningfully to the success of this project.

\;

\noindent Signed,

\noindent Prof. Arvind Easwaran

\noindent Professor, Nanyang Technological University (NTU)

==> contents/related_works.tex <==
\section{Related Works}
\label{sec:rel}


% This section discusses some of the recent works on the lane-keeping problem. \gao{Model-based control techniques like Model Predictive Control (MPC)~\cite{garcia1989model} and Rapidly-exploring Random Tree (RRT)~\cite{lavalle1998rapidly} have been applied to generic autonomous control task. MPC optimize state inputs to minimize a cost function~\cite{bujarbaruah2018adaptive, samuel2021lane}, while RRT explores feasible paths in an environment model~\cite{ma2014fast, lan2015continuous}.} % for shorter sentences in these less related works
% However, such techniques is heavy dependency on detailed state information or accurate system models, which may not be accessible in a real-world or model-free setting. Given such limitations, our work in this paper focuses on a model-free approach to the problem.


This section discusses some of the recent works on the lane-keeping problem. ~\citeauthor{garcia1989model}~\cite{garcia1989model} and \citeauthor{lavalle1998rapidly}~\cite{lavalle1998rapidly} proposed model-based control techniques like Model Predictive Control (MPC) and Rapidly-exploring Random Tree (RRT), respectively for any generic autonomous control task. MPC based methods optimize state inputs to minimize a cost function~\cite{bujarbaruah2018adaptive, samuel2021lane}. An RRT-based approach generates multiple feasible paths through incremental exploration using an environment model~\cite{ma2014fast, lan2015continuous}. However, a key limitation of such techniques is heavy dependency on detailed state information or accurate system models, which may not be accessible in a real-world or model-free setting. Given such limitations, our work in this paper focuses on a model-free approach to the problem.



%\textcolor{blue}{Model-based methods like Model Predictive Control (MPC)~\cite{garcia1989model} and Rapidly-exploring Random Tree (RRT)~\cite{lavalle1998rapidly}, are widely utilized for lane-keeping (LK) problem. MPC optimizing state inputs to minimize a cost function respecting objective functions~\cite{bujarbaruah2018adaptive, samuel2021lane} and RRT generating feasible paths through incremental exploration in the environment model~\cite{ma2014fast, lan2015continuous}. However, these methods depend heavily on detailed state information and accurate system models, which may not always be available in real-world settings or model-free environments like Duckietown, where only image inputs are available. Given these limitations, we mainly focus on model-free approaches rather than model-based ones.}

Currently, in many production vehicles, the lane-keeping features are integrated as a Level-2 (L2) autonomous driving standard. Such features are typically implemented through traditional approaches using lane detection and basic controllers~\cite{mccall2004integrated, jiang2010computer}.
%\textcolor{blue}{Current L2 autonomous driving production vehicles already include lane-keeping as a standard function, typically implemented through traditional approaches involving lane detection and basic controllers~\cite{mccall2004integrated, jiang2010computer, haque2019computer}.} 
These methods usually employ computer vision based control mechanism like OpenCV~\cite{bradski2000opencv} or Convolutional Neural Networks (CNNs)~\cite{lecun1998gradient} in combination with PID controllers~\cite{ziegler1942optimum}. 
While effective under ideal conditions, the performance of these systems can degrade significantly in challenging scenarios like sharp curves, adverse weather, or poor road visibility~\cite{rao2022developing}, potentially compromising navigation reliability and safety.

Alternatively, a learning-based sequential decision-making control mechanism delivers superior performance in complex driving scenarios, empowering the system to discern patterns and make the appropriate decisions. A typical learning-based solution to the LK problem falls under two categories --- supervised and reinforcement learning methods. An imitation learning-based approach called Behavior Cloning (BC)~\cite{ly2020learning, Mikita, pomerleau1988alvinn} is one of the popular supervised learning approaches. However, a fundamental limitation of the BC approach is that the model is trained offline on the scenarios and labeled data collected by an expert entity. This can lead to poor generalization beyond the demonstrated behaviors. Compounding error~\cite{ross2010efficient} is another well-known limitation of the BC method, as it does not explicitly account for the sequential nature of the LK problem. Small errors in a sequence of actions taken by the model compound over time.

% Compounding error~\cite{ross2010efficient} is another well-known limitation of the BC method, as it does not explicitly account for the sequential nature of the LK problem. Small errors in a sequence of actions taken by the model compound over time.
%Learning-based methods, aided by massive amounts of data, outperform \textcolor{blue}{L2 production techniques} in complex scenarios like sharp turns, enabling them to recognize patterns and make decisions in a broader context. A typical learning-based solution to the LK problem falls under two categories --- supervised and reinforcement learning-based methods. Imitation learning (supervised) based approach called Behavior cloning (BC) for lane-keeping has been applied in L3 automation~\cite{ly2020learning, Mikita, pomerleau1988alvinn}.\textcolor{blue}{ A key limitation of BC is the agent is trained offline on the scenarios and labeled data collected by the expert, leading to poor generalization beyond the demonstrated behaviors. For instance, if the expert consistently follows the optimal trajectory and never encounters situations where the car is near a boundary collision, the trained policy may struggle with how to avoid this collision when faced with such scenarios.} Compounding error~\cite{ross2010efficient} is another limitation of the BC method. As it does not explicitly account for the sequential nature of the LK problem, small errors in a sequence of actions taken by the agent compound over time. 

On the other hand, an RL-based approach can effectively tackle the challenges of generalizing to unseen scenarios and dealing with the sequential nature of the problem. This makes the RL-based approach especially essential as we progress towards higher levels of automation (L3, L4, and L5). \citeauthor{almasi2020robust} \cite{almasi2020robust} proposed an RL-based approach for the LK problem on the Duckietown framework. They use a na\"ive reward-shaping approach, in which the reward and cost functions are linearly combined and weighted by fixed coefficients. Other RL-based approaches also address the LK problem with fixed-weighted combinations for different objectives, such as minimizing the yaw angle~\cite{feher2018q, kHovari2020design}, crash avoidance~\cite{ashwin2023deep}, lateral and longitudinal control during lane changing~\cite{duan2020hierarchical}, etc.
However, a major limitation of the previous works is the weight coefficients in the modified reward definition are empirically selected, and these coefficient combinations may not be adaptive to different scenarios. 
% As mentioned in the previous section, the weight coefficients require tuning depending on the specific driving scenarios [xinwei: this is not the true, since they did not tuning.]

In our proposed method based on constrained RL, the weight coefficients for different objectives are learned appropriately, along with the agent's policy and its constraints. This alleviates the need for scenario-specific tuning of the weight coefficients. 
Additionally, this adaptable reward strategy enhances the RL agent’s lane-keeping reliability and overall driving effectiveness, making the agent more suitable for real-world autonomous driving applications.





% \aea{Where did this safety and reliability suddenly appear from? You never spoke about this earlier in the introduction. And why can't safety and reliability be achieved using weighted reward+cost functions?}


%\textcolor{blue}{which makes it particularly crucial as we move towards higher levels of automation (L4 and L5).} 
%Almasi et. al \cite{almasi2020robust} proposed an RL-based approach for the LK problem on the Duckietown framework. They use the na\"ive reward definition approach, where the reward and cost functions are linearly combined and weighted by fixed coefficients. 
%As highlighted in the previous section, the weight coefficients need tuning depending on the specific driving scenarios. Other RL-based approaches also address the LK problem with fixed-weighted combinations for different objectives, such as minimizing the yaw angle~\cite{feher2018q, kHovari2020design}, crash avoidance~\cite{ashwin2023deep}, lateral and longitudinal control during lane changing~\cite{duan2020hierarchical}, etc. \textcolor{blue}{However, a limitation of the previous works is the weight coefficients in the reward definition are arbitrarily selected, these coefficient combinations may not be adaptive in different scenarios.} In our proposed method based on constrained RL, the weight coefficients for different objectives are learned \textcolor{red}{appropriately} along with the agent's policy, \textcolor{red}{providing better performance on objectives of deviation elimination and collision avoiding compared with the previous fixed weight approach.} \textcolor{red}{ These constraints enforce safety and reliability in the learned driving policy, making the agent more suitable for real-world autonomous driving tasks, where maintaining certain lane discipline are crucial, as we observe in Section~\ref{sec:EvaluationofVariousScenarios}. Additionally, we perform extensive ablation studies on how different constraint parameters and learning rates affect the policy behavior. These constraint thresholds provide the trade-offs balance between safety and efficiency, as demonstrated in Section~\ref{sec:AblationStudy}.}

%We use \cite{almasi2020robust} as a baseline for comparison; empirically, we observe that the fixed-weight approaches perform sub-optimally in different driving scenarios when compared to our proposed method.
% A classical way to solve the LK problem is OpenCV~\cite{bradski2000opencv} based method~\cite{mccall2004integrated, jiang2010computer, haque2019computer}. The principle of these algorithms is using PID control to make vehicle movement based on the lanes detected by edge detection, color filtering, and geometric transformations. However, their effectiveness decreases substantially under conditions like sharp curves, varied weather, and poor road visibility, impacting navigation reliability and safety~\cite{rao2022developing}. 
% minimizing the reaching time in deep sea treasure~\cite{huang2017parameterized}, 
% speed tracking for smoothness consideration~\cite{ mannion2017policy}, 
%and by applying the Lagrange relaxation technique, we improve the policy performance compared with the fixed-weight approach.
%\aea{Is this the only RL based approach for AD? If so, this must be highlighted in the introduction to further strengthen the contributions.[Re: not only rl, but done]}

==> contents/requirement.tex <==
\section*{Requirement}

\textbf{1. Hardware (Provided by Presenter):}
\begin{itemize}
    \item \textbf{Duckiebot:} A fully operational Duckiebot equipped with:
    \begin{itemize}
        \item Jetson Nano for onboard computation.
        \item Camera for real-time visual input and processing.
        \item Motor control system for autonomous navigation.
    \end{itemize}
    \item \textbf{Duckietown Environment:} Portable Duckietown setup including:
    \begin{itemize}
        \item Modular tiles with lane markings for a 3x3 meter area.
        \item Obstacles for static and dynamic scenarios.
    \end{itemize}
    \item Power adapter and spare batteries for the Duckiebot.
\end{itemize}

\noindent\textbf{2. Software (Provided by Presenter):}
\begin{itemize}
    \item ROS (Robot Operating System) pre-installed on the Duckiebot.
    \item Python-based scripts for real-time control and monitoring.
    \item Constraint RL-trained policy for lane-keeping and obstacle avoidance tasks.
\end{itemize}

\noindent\textbf{3. Space Requirements:}
\begin{itemize}
    \item A demo area of at least 4x4 meters for setting up the Duckietown environment.
    \item A small table for the laptop and related accessories.
    \item Space for 1x1 meters near the demo area to store additional equipment (e.g., spare batteries, chargers, or Duckietown tiles).
\end{itemize}

\noindent\textbf{4. Power and Connectivity:}
\begin{itemize}
    \item Two standard power outlets for the Duckiebot charger and laptop.
    \item Reliable Wi-Fi connection for real-time communication between the laptop and Duckiebot.
\end{itemize}

\noindent\textbf{5. Display (Optional):}
\begin{itemize}
    \item A monitor or projector to display the Duckiebot's camera feed and analytics for audience engagement.
\end{itemize}

\noindent\textbf{6. Setup and Demo Time:}
\begin{itemize}
    \item Approximately 30 minutes to assemble the Duckietown environment and test the Duckiebot.
    \item Demo duration: 10-15 minutes per run, showcasing:
    \begin{itemize}
        \item Lane-keeping in small loop or zig-zag environment.
        \item Obstacle avoidance in dynamic environments.
    \end{itemize}
\end{itemize}

% \noindent\textbf{7. Safety Measures:}
% \begin{itemize}
%     \item An emergency stop function to halt the Duckiebot instantly if needed.
%     \item Visual indicators or low barriers around the demo area to ensure audience safety.
% \end{itemize}




==> figure/as_lr_table.tex <==
\begin{tabular}{@{\hspace{5mm}}c@{\hspace{5mm}}cccc}
\toprule
\multirow{2}{*}{$\eta_{3}$} & \multicolumn{4}{c}{$\eta_{1}=\eta_{2}$} \\
\addlinespace[1pt]
\cline{2-5}
\addlinespace[2pt]
 & $1e^{-3}$ & $1e^{-4}$ & $1e^{-5}$ & $1e^{-6}$ \\
 \midrule
 $1e^{-5}$ &  $C$ &  $C$ &  $C$ &  $C$ \\ 
 $1e^{-6}$ &  $NC$ &  $C$ &  $C$ &  $C$ \\
\bottomrule
% \addlinespace[1pt]
% \hlineB{2}
\end{tabular}



% \begin{tabular}{ccccccccc}
% % \toprule
% \hlineB{2}
% \addlinespace[2pt]
% \multirow{2}{*}{Map} & \multirow{2}{*}{Metric} & \multicolumn{7}{c}{Method} \\
% \cline{3-9}
% \addlinespace[2pt]
%  &  & \drcpo & \crcpo & \dppof & \cppof & \bl & \cbc  & \opencv  \\
% \midrule
% \multirow{4}{*}{Small loop} & Lane Distance Cost & 0.25$\pm$0.00 & 0.31$\pm$0.00 & 0.38$\pm$0.02 & 1.04$\pm$0.25 & 0.98$\pm$0.14 & 1.05$\pm$0.03 & 1.77\\
%                                 & Collision Cost & 0.05$\pm$0.00 & 0.05$\pm$0.01 & 0.06$\pm$0.00 & 0.34$\pm$0.20 & 0.37$\pm$0.00 & 0.46$\pm$0.06 & 0.98\\

%                                 & Total Step & 369.5$\pm$64.4 & 492.0$\pm$5.3 & 336.3$\pm$17.6 & 431.9$\pm$3.0 & 353.8$\pm$2.9 & 335.3$\pm$12.3 & 152.84\\
                                
%                                 & Travel Distance Reward & \textbf{69.1$\pm$0.6} & 62.4$\pm$22.2 & 46.5$\pm$3.3 & 51.3$\pm$14.8 & 50.2$\pm$2.6 & 55.7$\pm$1.7 & 14.79\\
% \midrule
% \multirow{4}{*}{Zig-zag} & Lane Distance Cost & 0.20$\pm$0.00 & 0.41$\pm$0.02 & 0.18$\pm$0.00 & 0.86$\pm$0.10 & 0.98$\pm$0.02 & 1.10$\pm$0.03 & 1.67\\
%                              & Collision cost & 0.05$\pm$0.00 & 0.06$\pm$0.00 & 0.05$\pm$0.00 & 0.24$\pm$0.08 & 0.41$\pm$0.05 & 0.56$\pm$0.08 & 0.95\\

%                             & Total Step & 404.5$\pm$27.2 & 482.9$\pm$0.5 & 369.9$\pm$2.6 & 453.0$\pm$0.0 & 346.9$\pm$9.9 & 310.6$\pm$22.6 & 168.97\\
                             
%                              & Total reward & \textbf{72.6$\pm$0.2} & 63.7$\pm$0.5 & 48.5$\pm$5.5 & 59.3$\pm$6.5 & 46.1$\pm$5.5 & 56.74$\pm$0.2 & 16.6\\
% \midrule
% \multirow{4}{*}{\makecell{Dynamic obstacle\\(Straight for OpenCV)}} & Lane Distance Cost & 0.20$\pm$0.00 & 0.41$\pm$0.02 & 0.18$\pm$0.00 & 0.86$\pm$0.10 & 0.98$\pm$0.02 & -- & \multicolumn{1}{c}{0.60}\\
%                              & Collision cost & 0.05$\pm$0.00 & 0.06$\pm$0.00 & 0.05$\pm$0.00 & 0.24$\pm$0.08 & 0.41$\pm$0.05 & -- & \multicolumn{1}{c}{0.34}\\

%                             & Total Step & \textbf{69.1$\pm$0.6} & 62.4$\pm$22.2 & 46.5$\pm$3.3 & 51.3$\pm$14.8 & 50.2$\pm$2.6 & -- & \multicolumn{1}{c}{443.0}\\
                             
%                              & Total reward & \textbf{72.6$\pm$0.2} & 63.7$\pm$0.5 & 48.5$\pm$5.5 & 59.3$\pm$6.5 & 46.1$\pm$5.5 & -- & \multicolumn{1}{c}{56.5}\\
% % \bottomrule
% \addlinespace[2pt]
% \hlineB{2}
% \end{tabular}










==> figure/discreteactionspace.tex <==
\begin{tabular}{lcc}
\hline
\textbf{Action} & \textbf{Left wheel} & \textbf{Right wheel} \\
\hline
turn-left & 0.04 & 0.4 \\
% \hline
turn-right & 0.4 & 0.04 \\
% \hline
go-straight & 0.3 & 0.3 \\
\hline
\end{tabular}

==> figure/hyper-parameters.tex <==
\begin{tabular}{lcl}
\toprule
\textbf{Parameters} & \textbf{Value} & \textbf{Description} \\
\midrule
$\eta$ & 2e-5 & Learning rate for gradient decent.\\
Runner & 4 & Parallel threads for data sampling.\\
$H$ & 512 & Batch size and the episode length.\\
$\gamma$& 0.95 &  Discount factor in RL.\\
$\epsilon$& 0.2 & Clip factor for PPO algorithm.\\
$\alpha_{1}$& 0.5 & Constrain threshold for lane deviation.\\
$\alpha_{2}$& 0.02 & Constrain threshold for collision.\\
$\alpha_{3}$& 0.01 & Constrain threshold for illegal driving.\\
reward factor& 10 & Gain for travel distance cost in reward.\\ 
lane factor& 100 & Gain for lane distance cost in reward.\\
collision factor& 40 & Gain for collision cost in reward.\\
illegal factor& 10 & Gain for illegal driving in reward.\\
Gradient clip& 10 & Gradient clip factor.\\
$\sigma$ clip& (0.2,0.6) & Actor variance boundary.\\
entropy factor& 0.001 & Entropy factor for policy gradient.\\
\bottomrule
\end{tabular}


==> figure/simple_loop.tex <==
\begin{tabular}{|c|c|c|c|c|}
\hline
\multirow{2}{*}{Approach} & \multicolumn{3}{c|}{Small loop map} \\
\cline{2-4}
 & Lane cost  & Collision cost &  Total reward\\
 \hline
\drcpo(Ours) & \textbf{0.25$ \pm$0.00} & \textbf{0.05$\pm$0.00} & \textbf{69.1$\pm$0.6}\\
\hline
\crcpo(Ours) & 0.31$\pm$0.00 & \textbf{0.05$\pm$0.01}&  62.4$\pm$22.2 \\
\hline
\dppof & 0.38$\pm$0.02 & 0.06$\pm$0.00 & 46.5$\pm$3.3\\
\hline
\cppof & 1.04$\pm$0.25 & 0.34$\pm$0.20 & 51.3$\pm$14.8\\
\hline
\bl & 0.98$\pm$0.14 & 0.37$\pm$0.00 & 50.2$\pm$2.6\\
\hline
\end{tabular}

% \begin{tabular}{|c|c|c|c|c|}
% \hline
% \multirow{2}{*}{Approach} & \multicolumn{4}{c|}{Small loop map} \\
% \cline{2-5}
%  & Lane cost  & Coll. cost & Srv. steps &  Tot. reward\\
%  \hline
% \drcpo & \textbf{0.25$ \pm$0.00} & \textbf{0.05$\pm$0.00} & 431.9$\pm$3.0 & \textbf{69.1$\pm$0.6}\\
% \hline
% \crcpo & 0.31$\pm$0.00 & \textbf{0.05$\pm$0.01}& \textbf{492.0$\pm$5.3} & 62.4$\pm$22.2 \\
% \hline
% \dppof & 0.38$\pm$0.02 & 0.06$\pm$0.00 & 336.3$\pm$17.6 & 46.5$\pm$3.3\\
% \hline
% \cppof & 1.04$\pm$0.25 & 0.34$\pm$0.20 & 369.5$\pm$64.4 & 51.3$\pm$14.8\\
% \hline
% \bl & 0.98$\pm$0.14 & 0.37$\pm$0.00 & 353.8$\pm$2.9 & 50.2$\pm$2.6\\
% \hline
% \end{tabular}

==> figure/tab_sl_zz.tex <==
\begin{tabular}{ccccccccc}
% \toprule
\hlineB{2}
\addlinespace[2pt]
\multirow{2}{*}{\textbf{Scenarios}} & \multirow{2}{*}{\textbf{Metrics}} & \multicolumn{3}{c}{\textbf{Discrete Methods}} & \multicolumn{4}{c}{\textbf{Continuous Methods}} \\
% \cline{3-5} \cline{6-9}
\cmidrule(rl){3-5} \cmidrule(rl){6-9}
\addlinespace[2pt]
 &  & \drcpo & \dppof & \bl~\cite{bellman1952theory} & \crcpo & \cppof & \cbc~\cite{bertesekas1999nonlinear} & \opencv~\cite{chen2020lane}  \\
\midrule
\multirow{3}{*}{Small loop} & Lane Deviation Cost & {0.66$\pm$0.02} & 0.99$\pm$0.07 & 0.98$\pm$0.14 & \textbf{0.31$\pm$0.00} & 1.04$\pm$0.25 & 0.79$\pm$0.02 & 1.65$\pm$0.16\\
                                & Collision Cost & {0.17$\pm$0.00} & 0.38$\pm$0.04 & 0.37$\pm$0.00 & \textbf{0.05$\pm$0.01} & 0.34$\pm$0.20 & 0.17$\pm$0.00 & 0.88$\pm$0.14\\
                                & Travel Distance Reward & \textbf{69.0$\pm$0.6} & 46.6$\pm$3.2 & 50.2$\pm$2.6 & {62.4$\pm$22.2} & 51.3$\pm$14.8 & 43.8$\pm$0.0 & 18.4$\pm$5.1\\
\midrule
\multirow{3}{*}{Zig-zag} & Lane Deviation Cost & {0.57$\pm$0.04} & 0.82$\pm$0.08 & 0.98$\pm$0.02 & \textbf{0.41$\pm$0.02} & 0.86$\pm$0.10 & 0.77$\pm$0.02 & 1.60$\pm$0.10\\
                             & Collision Cost & {0.12$\pm$0.00} & 0.31$\pm$0.02 & 0.41$\pm$0.05 & \textbf{0.06$\pm$0.00} & 0.24$\pm$0.08 & 0.16$\pm$0.04 & 0.87$\pm$0.12\\
                             & Total Distance Reward & \textbf{72.6$\pm$0.1} & 52.3$\pm$6.2 & 46.1$\pm$5.5 & {63.7$\pm$0.5} & 59.3$\pm$6.5 & 49.7$\pm$1.0 & 19.3$\pm$3.8\\
\midrule
\multirow{3}{*}{\makecell{Dynamic obstacle}} & Lane Deviation Cost & {0.63$\pm$0.15} & 0.88$\pm$0.00 & 0.93$\pm$0.18 & \textbf{0.38$\pm$0.08} & 0.64$\pm$0.19 & 0.77$\pm$0.06 & --\\
                             & Collision Cost & {0.32$\pm$0.05} & 0.47$\pm$0.09 & 0.78$\pm$0.12 & \textbf{0.20$\pm$0.08} & 0.33$\pm$0.06 & 0.48$\pm$0.04 & --\\
                             & Total Distance Reward & {68.8$\pm$4.1} & 45.1$\pm$5.6 & 33.0$\pm$5.7 & \textbf{82.0$\pm$16.4} & 63.0$\pm$24.1 & 57.1$\pm$1.0 & --\\
\addlinespace[2pt]
\hlineB{2}
\end{tabular}




==> figure/tableresultcontinuous.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Continuous} & \multicolumn{4}{c|}{Simple Loop} & \multicolumn{4}{c|}{Zigzag} \\
\cline{2-9}
 & Cost Lane & Cost Coll & Total Step & Total Reward & Cost Lane & Cost Coll & Total Step & Total Reward \\
\hline
Fixed & 0.98 & 0.29 & 378.90 & 65.25 & - & - & - & - \\
\hline
RCPO & 0.34 & 0.04 & 492.24 & 70.49 & 0.43 & 0.06 & 483.28 & 64.08 \\
\hline
\end{tabular}



==> figure/tableresultdiscrete.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Approach} & \multicolumn{4}{c|}{Simpleloop} & \multicolumn{4}{c|}{Zigzag} \\
\cline{2-9}
 & Cost Lane & Cost Coll & Total Step & Total Reward & Cost Lane & Cost Coll & Total Step & Total Reward \\
\hline
Fixed & 0.37 & 0.06 & 348.71 & 48.85 & 0.18 & 0.05 & 371.76 & 44.62 \\
\hline
RCPO & 0.26 & 0.05 & 429.75 & 68.66 & 0.24 & 0.05 & 434.00 & 69.18 \\
\hline
\end{tabular}


==> figure/zigzag.tex <==
\begin{tabular}{|c|c|c|c|c|}
\hline
\multirow{2}{*}{Approach} & \multicolumn{3}{c|}{Zig-zag map} \\
\cline{2-4}
 & Lane cost  & Collision cost & Total reward\\
\hline
\drcpo(Ours) & 0.20$\pm$0.00 & \textbf{0.05$\pm$0.00} &  \textbf{72.6$\pm$0.2} \\
\hline
\crcpo(Ours) & 0.41$\pm$0.02 & 0.06$\pm$0.00 &  63.7$\pm$0.5\\
\hline
\dppof & \textbf{0.18$\pm$0.00} & \textbf{0.05$\pm$0.00} & 48.5$\pm$5.5\\
\hline
\cppof & 0.86$\pm$0.10 & 0.24$\pm$0.08 &  59.3$\pm$6.5\\
\hline
\bl & 0.98$\pm$0.02 & 0.41$\pm$0.05 &  46.1$\pm$5.5\\
\hline
\end{tabular}


% \begin{tabular}{|c|c|c|c|c|}
% \hline
% \multirow{2}{*}{Approach} & \multicolumn{4}{c|}{Zig-zag map} \\
% \cline{2-5}
%  %& Lane cost  & Coll. cost & Travel Steps & Reward\\
%  & Lane cost  & Coll. cost & Srv. steps &  Tot. reward\\
% \hline
% \drcpo & 0.20$\pm$0.00 & \textbf{0.05$\pm$0.00} & 453.0$\pm$0.0 & \textbf{72.6$\pm$0.2} \\
% \hline
% \crcpo & 0.41$\pm$0.02 & 0.06$\pm$0.00 & \textbf{482.9$\pm$0.5} & 63.7$\pm$0.5\\
% \hline
% \dppof & \textbf{0.18$\pm$0.00} & \textbf{0.05$\pm$0.00} & 369.9$\pm$2.6 & 48.5$\pm$5.5\\
% \hline
% \cppof & 0.86$\pm$0.10 & 0.24$\pm$0.08 & 404.5$\pm$27.2 & 59.3$\pm$6.5\\
% \hline
% \bl & 0.98$\pm$0.02 & 0.41$\pm$0.05 & 346.9$\pm$9.9 & 46.1$\pm$5.5\\
% \hline
% \end{tabular}
